Terrain-Aware Quadrupedal Locomotion via Reinforcement Learning

In nature, legged animals have developed the ability to adapt to challenging terrains through perception, allowing them to plan safe body and foot trajectories in advance, which leads to safe and energy-efficient locomotion. Inspired by this observation, we present a novel approach to train a Deep Neural Network (DNN) policy that integrates proprioceptive and exteroceptive states with a parameterized trajectory generator for quadruped robots to traverse rough terrains. Our key idea is to use a DNN policy that can modify the parameters of the trajectory generator, such as foot height and frequency, to adapt to different terrains. To encourage the robot to step on safe regions and save energy consumption, we propose foot terrain reward and lifting foot height reward, respectively. By incorporating these rewards, our method can learn a safer and more efficient terrain-aware locomotion policy that can move a quadruped robot flexibly in any direction. To evaluate the effectiveness of our approach, we conduct simulation experiments on challenging terrains, including stairs, stepping stones, and poles. The simulation results demonstrate that our approach can successfully direct the robot to traverse such tough terrains in any direction. Furthermore, we validate our method on a real legged robot, which learns to traverse stepping stones with gaps over 25.5cm.

==> ICRA_revise/Review1.tex <==
Reviewer 1 of ICRA 2023 submission 2505

Comments to the author
======================

The submission proposes a DNN-adjusted trajectory generator
as a controller of quadrupedal locomotion that observes the
controlled robot's dynamic state and the surrounding
terrain. The authors argue that providing the terrain
information to the controller results in 'safer' and 'more
efficient' control policies. The subject is relevant in the
field, and the capability for the robust traversal of
discontinuous terrain is crucial; however, the paper needs
more care in its writing, especially in the evaluation's
rigor. Nevertheless, it could be great with an overhaul and
a later resubmission.

The two main aspects of the contribution, 'safety' and
'efficiency,' do not gain specific meaning until the
discussion of results, from where one can reverse-engineer
them. The definition of 'safety' is not intuitive,
'robustness' would have been a better term. The
presentation of the success rate is hard to understand; the
relevant parts could have gotten more emphasis, e.g., it
would have been beneficial to present the calculation as an
equation. How much was the maximum possible distance the
robot could travel per direction? Is there a trade-off
between a higher velocity and robustness?

As I understand, the controller was trained in simulation
and then transferred to the real world; I would have
appreciated an examination of the transfer's quality,
however preliminary it might have been. E.g., how do the
success rates fare in reality against those from
simulation? How much of the robustness is lost?

The paper addressing the aspect of 'efficiency' is
exemplary; it would benefit the paper to emphasize it more
explicitly. E.g., in the last sentence in Section I
paragraph 3, the authors write that other solutions do not
address efficiency; what are some specific aspects that
show this in the other solutions? E.g., legs controlled to
their maximum height. Also, 'efficiency' needs to be more
apparent in the metrics. For example, while a
not-overcontrolled actuator should consume less power, how
does this translate into running time or battery life? Is
the power consumption of the training significant?

To my knowledge, the LSTM network is not a recent
technology. Is there a reason behind the choice? Have other
structures been considered? Overall, the paper could have
reflected more on other related work. For example, several
references are presented in Section II-A, but only [1] and
[5] are reflected. Also, in this Section, the authors argue
that it is a bottleneck that other solutions rely heavily
on the accuracy of the dynamical model for model-based
control. How does the proposed solution address this
specifically? Also, is the PID controller that applies the
motor torques based on the position reference signal
modeled in the simulation? How was the PID controller
synthesized?

In Section II-C, the authors reflect on solutions
exploiting visual data to traverse rough terrain. It would
have been great to learn how the proposed solution using
the offline landscape map compares. For example, how do the
authors see the map generated for new areas?

In general, mathematical formalism is not used to the
reader's benefit. The ideas and considerations behind their
application are often missing, the usage and definition of
symbols are generally confusing, and the distinction
between vectors and scalars could be more apparent. E.g., a
sentence per reward component on what the authors aimed to
bias the solution towards would have been greatly
appreciated.

Overall, the paper would greatly benefit from a more
rigorous evaluation, a more precise presentation of
results, and a more solid placement in its
state-of-the-art. Therefore, I recommend a rejection now
and later resubmission.

Comments on the Video Attachment
================================

It is always great to see the results working; I would have
appreciated seeing more real-world experiments. I also feel
that too many things are presented simultaneously; it is
easy to lose focus, especially on the simulations.

==> ICRA_revise/Review2.tex <==
Reviewer 2 of ICRA 2023 submission 2505

Comments to the author
======================

They incorporate both proprioceptive and exteroceptive
information for safe and energy-efficient quadrupedal
locomotion using deep RL in simulation on rough discrete
terrains. 
It can traverse over block terrains, stairs, stepping
stones with 
gaps, and poles while being safer and more energy-efficient
in any
direction. They show that the real robot can traverse
stepping stones with gaps up to 25cm.

The contribution consists in using both proprioceptive and
exteroceptive as inputs of a DNN (LSTM trained with PPO) to
adjust a trajectory generator to promote safe control and
energy efficiency. They are the first fully learning-based
method to use both. Previous methods did not consider
energy efficiency (while their method adapts the stepping
height to do so) and did not adopt the x/y positioning of
the feet which prevent them from traversing poles and
stepping stones. 

Strength: 
- Successful experiments on the real robot 
- Several experiments on simulation on 4 different terrains
- Comparison to two other methods: only proprioceptive
information and fixed trajectory 
- Seek energy efficiency 
- Their method is clearly explained

Weakness:
- The results are more qualitative than quantitative (there
is no statistical comparison)
- saying that model-based methods require experts knowledge
is true but they simply shift the expert knowledge of using
model-based methods with expert knowledge of using DRL,
reward shaping for example (which can be easier to acquire
nowadays) 
- for the real robot they use mocap to compute the robot's
position and an offline map to deduce the height map. How
do they plan to deploy it in a real-world scenario, knowing
for example that frontal cameras often present in
quadrupedal robots do not offer a view of the surrounding
of the feet?

Minor corrections:
- add descriptions of what are d_l, c_x, and c_y in
equations 4, 5, and 6 
- better explain how many runs there are for the
comparison: is there only one trained model evaluated on 3
seeds * 6 directions on the four environments, or one model
for each environment/direction? And add statistical
comparisons (using the values presented in figure 4) to
present thorough quantitative results. 
- better explain what is there to see in Figure 6 (maybe
add annotation along the time axis to show when the robot
is traversing each gap)


Comments on the Video Attachment
================================

It shows the efficiency of their method on the simulated
four terrains, the comparison to the other methods for
climbing stairs, and two successful deployments on the real
robot. (note: it seems to have been recorded on 16/9 but
squished to 4/3). 

==> ICRA_revise/Review3.tex <==
Reviewer 9 of ICRA 2023 submission 2505

Comments to the author
======================

The paper presents a method to generate policies that use
exteroceptive and proprioceptive information to traverse
challenging terrain. To do so in a safe way, they propose
using a trajectory generator to make learning safer and
easier. They evaluate their work on 4 sets of tasks -
block, stair, stepping stones and poles. The method is
compared against two baselines: A policy with only
proprioceptive data, and a policy that uses a fixed TG.
They show that their method on their tasks perform better
than the baselines and also show it working on the actual
robot.



In my understanding the paper is very similar to the
teacher policy in [1], but with a few differences
Similarity:

The policy (teacher policy in [1]) has access to terrain
profile (exteroceptive information)

Uses a similar TG to generate reference trajectories
Trained against randomized terrain



Important Differences:
[1] (Teacher policy) uses a policy based leg frequency
conditioned TG to generate a trajectory that only varies
the foot’s location in the z axis, then adds policy based
residuals in the foot position, and then calculates the
joint angles using an IK solver

The authors use a policy based leg frequency and foot
height conditioned TG to generate a trajectory that varies
the foot location in 3d space, then use an IK solver to get
desires joint angles, and then add policy based residuals
in the joint space
 

In [1], the MLP based teacher policy (that has both
proprioceptive and exteroceptive information) is distilled
into a TCN student policy that only has sequential
proprioception, and deploys the student policy on the real
robot

The authors train a single LSTM policy that has both
proprioception and exteroception, that is deployed in the
real robot. 



Major comments:

The authors present a method that is very similar to [1]
but with a few potentially meaningful changes. But they do
not accurately baseline their method with [1]. Rather they
use a component of [1], the fixed FTG, and use it with
their method as a baseline. This is an unfair baseline as
the TG in [1] is fixed because their policy provides
residuals in the foot’s position, while the policy here
only provides the residuals in the joint space after using
an IK solver. The other baseline is their method without
exteroception.
The idea of using a policy estimated foot height TG was
done in [2]. The idea of using exteroception to train
quadruped policies for varying terrain has also been done
recently in [3]. 
Since this work draws inspiration from
[1],[2],[3], I believe that the authors should incorporate
a stronger set of baselines to show how their method
compares.

The method introduced is an end to end learning based
approach, and therefore we cannot draw any theoretical
conclusions on the safety of the policy. In the absence of
this, the authors should show their results across multiple
seeds (as done in [1]).


Minor comments:

The plots in Fig 6 (b) are not legible

All these points weaken the possible contribution of the
paper and should be carefully considered by the authors in
their future developments.



References:
[1] J. Lee, J. Hwangbo, L. Wellhausen, V. Koltun, and M.
Hutter, “Learning quadrupedal locomotion over challenging
terrain,” Science robotics, vol. 5, no. 47, p. eabc5986,
2020.
[2] Iscen, Atil, Ken Caluwaerts, Jie Tan, Tingnan Zhang,
Erwin Coumans, Vikas Sindhwani, and Vincent Vanhoucke.
"Policies modulating trajectory generators." In Conference
on Robot Learning, pp. 916-926. PMLR, 2018.
[3] Rudin, Nikita, David Hoeller, Philipp Reist, and Marco
Hutter. "Learning to walk in minutes using massively
parallel deep reinforcement learning." In Conference on
Robot Learning, pp. 91-100. PMLR, 2022.


Comments on the Video Attachment
================================

The video illustrates well the approach.

==> ICRA_revise/Review4.tex <==
Reviewer 14 of ICRA 2023 submission 2505

Comments to the author
======================

This paper presents a terrain aware quadruped locomotion.

It uses both exteroception and proprioception to walk over
stairs, gaps or stepping stones in simulation, and walked
over a gap with the real robot.

Although the motion in simulation was smooth and some real
world experiment was shown, the novelty of this work was
not properly written in the paper.

The main contribution of this paper is written as 

1) We propose a deep reinforcement learning framework with
a parameterized trajectory generator that integrates both
the proprioceptive and exteroceptive
information.

And the method it used was a height scan around each foot
as the exteroceptive input and combining it with a
recurrent neural network .

However this is almost identical to the related work by
[14], and this was not mentioned at all in the method
section. The author cited [8] for the trajectory generator
but didn’t cite any previous work for observation or reward
even though it is almost identical to [8] or [14].

For example, the height scan pattern is the same as [14]
but not referenced in the text.

The only major difference in the method is that the policy
changes the xyz position and height of the trajectory
generator at the same time with residual joint position
target. 

The action space in [8] is phase difference (4) + xyz
residual (12).
The action space in [14] is phase difference (4) + joint
residual (12).
This work’s action space seems to be phase difference(4) +
xyz residual (12) + height residual (4) + joint residual
(12).

Therefore the explanation in the text,
”Compared with the TG in [8], our parameterized TG is
capable of adjusting the foot height by adding &#948; h
from the DNN policy, and it also provides the movement in
XY plane dx, dy, where [8] only considers the movement in
the Z-axis.” is not precise.

This also makes the comparison result not fair since the
“fixed TG” only changes z.

Also during the real robot experiment, the robot used
motion capture data with the offline map to acquire the
exteroception data. This limits the applicability of the
method to be used in the real world environment.


[8] J. Lee, J. Hwangbo, L. Wellhausen, V. Koltun, and M.
Hutter,
“Learning quadrupedal locomotion over challenging terrain,”
Science
robotics, vol. 5, no. 47, p. eabc5986, 2020.
[14] T. Miki, J. Lee, J. Hwangbo, L. Wellhausen, V. Koltun,
and M. Hutter,
“Learning robust perceptive locomotion for quadrupedal
robots in the
wild,” Science Robotics, vol. 7, no. 62, p. eabk2822, 2022.

Comments on the Video Attachment
================================

The video shows the motion of the robot clearly.
